Using Mise-En-Sc\`ene Visual Features based on MPEG-7 and Deep Learning for Movie Recommendation

Item features play an important role in movie recommender systems, where recommendations can be generated by using explicit or implicit preferences of users on traditional features (attributes) such as tag, genre, and cast. Typically, movie features are human-generated, either editorially (e.g., genre and cast) or by leveraging the wisdom of the crowd (e.g., tag), and as such, they are prone to noise and are expensive to collect. Moreover, these features are often rare or absent for new items, making it difficult or even impossible to provide good quality recommendations. In this paper, we show that user's preferences on movies can be better described in terms of the mise-en-sc\`ene features, i.e., the visual aspects of a movie that characterize design, aesthetics and style (e.g., colors, textures). We use both MPEG-7 visual descriptors and Deep Learning hidden layers as example of mise-en-sc\`ene features that can visually describe movies. Interestingly, mise-en-sc\`ene features can be computed automatically from video files or even from trailers, offering more flexibility in handling new items, avoiding the need for costly and error-prone human-based tagging, and providing good scalability. We have conducted a set of experiments on a large catalogue of 4K movies. Results show that recommendations based on mise-en-sc\`ene features consistently provide the best performance with respect to richer sets of more traditional features, such as genre and tag.

==> cbrs.tex <==
\subsection{Content-Based Recommender Systems}

Content-based RSs   model preferences of a user exploiting the   content of items and feedbacks provided by the user to the items.
 Feedbacks could be obtained either by explicitly requesting the users ~\cite{billsus1999hybrid}, or implicitly by analyzing her activity~\cite{kelly2003implicit}. Recommendations are then generated by matching the user model against the features of entire item catalog. 
 
Content of items is typically described by textual features and is modeled by Vector Space Model (VSM), i.e., a model that represents an item as a vector in a multi-dimensional space. These dimensions represent the features used to describe the items. By means of this representation, the system measures a relevance score that represents the user's degree of interest toward any of these items~\cite{lops2011content}. For instance, in the movie domain, the features that describe an item can be genre, actors, or director~\cite{de2015semantics,musto2012enhanced}. 
%This model may allow content-based recommender systems to naturally tackle the new item problem~\cite{elahi2013active}. Other families of content-based RSs use semantic analysis (lexicons and ontologies) to create more accurate item representations~\cite{degemmis2007content,eirinaki2003sewep,magnini2001improving}.

There are already a variety of content-based recommendation aproaches proposed. A  classical example is the  k-nearest neighborapproach (KNN) that computes the preference of a user for an unknown item by comparing it against all the items known by the user in the catalogue. Every known item contributes to predict the preference score according  to its similarity with the unknown item. The similarity can be measured by typically using   Cosine similarity     ~\cite{lops2011content,Pazzani07CRS}. 
%There are also works that model the probability for the user to be interested to an item using a Bayesian approach   ~\cite{mooney2000content}, or use other techniques adopted from IR (Information Retrieval) such as the Relevance Feedback method~\cite{ahn2007open}.


==> method-cbf.tex <==
% \subsubsection{Content-Based Filtering}
% We adopt a classical ``$k$-nearest neighbours'' content-based algorithm \cite{cremonesi2012user}. 
% %\cite{lops2011content} 
% Given a set of users $u \in U$ and a catalogue of items $i \in I$, $r_{ui} \in R$ is the rating given by user $u$ to item $i$ ($r_{ui} = 0$ if no rating is available). 
% Moreover, each item $i$ is associated to its feature vector $f_i \in F$. 
% For each pair of items $i$ and $j$, the similarity score $s_{ij} \in S$ is computed using the cosine of the corresponding feature vectors.
% \begin{equation}
% s_{ij} = \frac{\boldsymbol{f_i}^T\boldsymbol{f_j}}{{\boldsymbol{||f_i||}}{\boldsymbol{||f_j||}}+\text{shrink}}
% \end{equation}
% where \emph{shrink} is a parameter used to control support and it is tuned via cross validation.
% %
% %\begin{equation}
% %s_{ij} = \frac{\boldsymbol{f_i}^T\boldsymbol{f_j}}{\norm{\boldsymbol{f_i}}\norm{\boldsymbol{f_j}}}
% %\end{equation}
% For each item $i$, $\text{NN}_i$ is the set of its $k$-nearest neighbors. 
% The predicted rating ${\hat{r}_{ui}}$ of user $u$ on item $i$ is computed as 
% \begin{equation}
% 	{\hat{r}_{ui}} = \frac{\sum_{j \in \text{NN}_i, r_{uj} > 0}{r_{uj}s_{ij}}}{\sum_{j \in \text{NN}_i, r_{uj} > 0}{s_{ij}}}
% \end{equation}


==> table1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[tp]
\centering
 \caption{Comparison of aggregation functions for MPEG-7 and DNN features}
\label{my-label}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline 
Algorithm & Aggregation  & Recall          & Precision       & MAP \\ 
          &              & @10             & @10             & @10 \\ \hline
MPEG7 SCD & intersection & \textbf{0.0221} & 0.0045          &  \textbf{0.0071} \\  
MPEG7 SCD & union        &  0.0215         & \textbf{0.0048} & 0.0068  \\  
MPEG7 SCD & average      & 0.0197          & 0.0043          & 0.0063  \\  
MPEG7 SCD & median       & 0.0191          & 0.0041          & 0.0063  \\ \hline
MPEG7 HTD & intersection & \textbf{0.0232} & \textbf{0.0048} & \textbf{0.0083} \\  
MPEG7 HTD & union        & 0.0180          & 0.0040          & 0.0056   \\  
MPEG7 HTD & average      & 0.0198          & 0.0043          & 0.0067  \\  
MPEG7 HTD & median       & 0.0205          & 0.0042          & 0.0063   \\ \hline
MPEG7 EHD & intersection & \textbf{0.0550} & \textbf{0.0105} & \textbf{0.0205}  \\ 
MPEG7 EHD & union        & 0.0200          & 0.0043          & 0.0069   \\ 
MPEG7 EHD & average      & 0.0208          & 0.0046          & 0.0070   \\ 
MPEG7 EHD & median       & 0.0210          & 0.0043          & 0.0067   \\ \hline
MPEG7 CSD & intersection & \textbf{0.0299} & \textbf{0.0057} & \textbf{0.0109} \\ 
MPEG7 CSD & union        & 0.0209          & 0.0047          & 0.0067  \\  
MPEG7 CSD & average      & 0.0198          & 0.0042          & 0.0068   \\  
MPEG7 CSD & median       & 0.0195          & 0.0043          & 0.0066   \\ \hline
MPEG7 CLD & intersection & 0.0210          & 0.0044          & 0.0065  \\  
MPEG7 CLD & union        & 0.0214          & 0.0047          & 0.0073   \\  
MPEG7 CLD & average      & \textbf{0.0221} & \textbf{0.0049} & \textbf{0.0082}  \\  
MPEG7 CLD & median       & 0.0209          & 0.0045          & 0.0067   \\ \hline
DNN & intersection       & 0.0198          & 0.0042          & 0.0064  \\ 
DNN & union              & 0.0203          & 0.0046          & 0.0064   \\ 
DNN & average            & \textbf{0.0216} & 0.0046          & \textbf{0.0067}   \\ 
DNN & median             & 0.0205          & 0.0045          & 0.0066   \\ \hline
\end{tabular}%
%}
\label{tbl:results}
\end{table}

